Provably Optimal Memory Capacity for Modern Hopfield Models: Transformer-Compatible Dense Associative Memories as Spherical Codes

We study the optimal memorization capacity of modern Hopfield models and Kernelized Hopfield Models (KHMs), a transformer-compatible class of Dense Associative Memories. We present a tight analysis by establishing a connection between the memory configuration of KHMs and spherical codes from information theory. Specifically, we treat the stored memory set as a specialized spherical code. This enables us to cast the memorization problem in KHMs into a point arrangement problem on a hypersphere. We show that the optimal capacity of KHMs occurs when the feature space allows memories to form an optimal spherical code. This unique perspective leads to: (i) An analysis of how KHMs achieve optimal memory capacity, and identify corresponding necessary conditions. Importantly, we establish an upper capacity bound that matches the well-known exponential lower bound in the literature. This provides the first tight and optimal asymptotic memory capacity for modern Hopfield models. (ii) A sub-linear time algorithm $\mathtt{U}\text{-}\mathtt{Hop}$+ to reach KHMs' optimal capacity. (iii) An analysis of the scaling behavior of the required feature dimension relative to the number of stored memories. These efforts improve both the retrieval capability of KHMs and the representation learning of corresponding transformers. Experimentally, we provide thorough numerical results to back up theoretical findings.

==> background.tex <==
Give a set of memories $\bm{\Xi}$, and a query $\bx$.
The Hopfield network retrieves a pattern by iteratively updating the query $x^{(t)} \rightarrow x^{(t+1)}$ with its update rule for some $t \in \{0,1,... \}$.
This update rule eventually converges to a fixed point $\bx^\star$.
The fixed point $\bx^\star$ can either match one of the memories or the mixture thereof.
The update rule also corresponds to the minimization of an energy function $E(\bx)$ and the fixed point $\bx^\star$ is the local minima of $E(\bx)$.
Different selection of update rules and the corresponding energy function results in different memory capacity.
For example, a type of modern Hopfield networks as introduced in \cite{ramsauer2020hopfield} (detailed described in \cref{background:MHN}), enjoys a memory capacity exponential in $d$.



\subsection{Uniform Hopfield Memory}
\label{sec:kernel}

As described in \cref{background:MHN}, modern Hopfield Networks are capable of storing exponential many memories and retrieve them with small error.
The retrieval process consists of two steps.
First, calculating the memory-query overlap with some similarity measure.
Second, normalize or scale the similarities into weights to retrieve each memory w.r.t. the weight through linear combination.
However, the retrieval accuracy and memory capacity highly depends on the memory pattern geometry.
To retrieve the $\mu$-th memory, one requires large separation, which is defined by $\Delta_\mu \coloneqq \Braket{ \bxi_\mu, \bxi_\mu } - \underset{\nu,\nu\neq\mu}{\max} \Braket{\bxi_\nu, \bxi_\mu}$.

Recently, \cite{wu2024uniform} showed one is able to use a linear kernel $\calK$ as the similarity measure $\Phi \coloneqq \R^d \rightarrow \R^{D_\Phi}$.
The kernelized Hopfield Networks (KHNs) have the following update rule:
\begin{equation}\label{KHN-update-rule}
   \bx^{t+1} \leftarrow \calT_\Phi( \bx^t )
   =
   \bm{\Xi}
   \cdot
   Norm
   \(
   \beta
   \calK( \bm{\Xi}, \bx )
   \),
\end{equation}
where $\calK( \bm{\Xi}, \bx ) = \[ \calK( \bxi_\mu, \bx ) \]_{\mu=1}^M = \[  \Braket{\Phi(\bxi_\mu),  \Phi(\bx)} \]_{\mu=1}^M$.
Note that such construction preserves defining properties of MHNs such as fixed point convergence \cite[~Lemma 2.1]{wu2024uniform} and energy minimization \cite[~Theorem 2.1]{wu2024uniform}.
With this construction, accurate retrieval and large capacity are no longer depend on $\Delta_\mu$, but now depend on $\Delta_\mu^\Phi \coloneqq \calK( \bxi_\mu, \bxi_\mu ) - \underset{\nu,\nu\neq\mu}{\max} \calK( \bxi_\mu, \bxi_\nu )$.
Notably, the term $\Delta_\mu^\Phi$ is determined by $\Phi$.
In the case of $\Phi(\bx) = \bW \bx$, $\bW \in \R^{d \times D_\Phi}$, the term $\Delta_\mu^\Phi$ can be maximized via gradient descent on $\bW$.


We follow \cite{wu2024uniform, ramsauer2020hopfield} to define the memory storage and retrieval as:
\begin{definition}[Pattern Stored and Retrieved]
\label{def:stored_and_retrieved}
For all $\mu\in[M]$, let $R_\Phi\coloneqq \half \Min_{\nu\neq \mu;\nu,\mu\in[M]}\norm{\Phi(\bxi_\mu)-\Phi(\bxi_\nu)}$ be the finite radius 
 of each sphere $\calS_{\Phi,\mu}$ centered at memory pattern $\Phi(\bxi_\mu)$ in the feature space.
We say $\bxi_\mu$ is \textit{stored} if there exists a fixed point of $\calT_\calK$, such that $\Phi(\bx^\star_\mu) \in \calS_{\Phi,\mu}$, to which all limit points $\Phi(\bx) \in \calS_{\Phi,\mu}$ converge to, and $\calS_{\Phi,\mu} \cap \calS_{\Phi,\nu}=\emptyset$ for $\nu \neq \mu$. 
We say $\bxi_\mu$ is $\epsilon$-\textit{retrieved} by $\calT_\calK$ with $\bx$ for an error $\epsilon$.
\end{definition}
Note that this definition is compatible with both KHNs and MHNs (with identity feature map).













































    








